Studying Maximum Information Leakage Using Karush-Kuhn-Tucker Conditions

When studying the information leakage in programs or protocols, a natural question arises: "what is the worst case scenario?". This problem of identifying the maximal leakage can be seen as a channel capacity problem in the information theoretical sense. In this paper, by combining two powerful theories: Information Theory and Karush-Kuhn-Tucker conditions, we demonstrate a very general solution to the channel capacity problem. Examples are given to show how our solution can be applied to practical contexts of programs and anonymity protocols, and how this solution generalizes previous approaches to this problem.

==> eptcsdata.tex <==
\providecommand{\event}{M. Boreale, S. Kremer (Eds.):\\
 Security Issues in Concurrency (SecCo'09)}
\providecommand{\volume}{7}
\providecommand{\anno}{2009}
\providecommand{\firstpage}{1}
\providecommand{\eid}{1}
\pdfoutput=1

